Elasticity Solver in Minecraft for Learning Mechanics of Materials by Gaming

Video games have emerged as a medium for learning by creating engaging environments, encouraging creative and deep thinking, and exposing learners to complex problems. Unfortunately, even though there are increasing examples of video games for many basic science and engineering concepts, similar efforts for higher level engineering concepts such as mechanics of materials are still lacking. Here we present a mesh-free elasticity solver implementation in the popular video game Minecraft, a sandbox game where players can build any structure they can imagine. Modifications to the game, called mods in the Minecraft community, are a common feature of this platform. Our elasticity mod computes the stress and deformation of arbitrary structures and colors the blocks with a heat-map to visualize the result of the analysis. We used this mod in the Honors section of two courses taught at Purdue University: Basic Mechanics I Statics, Mechanics of Materials. This articles describes our experience developing and deploying this tool to encourage its use in biomedical engineering classrooms. A future goal is to engage the broader audience Minecraft players that already interact regularly with Minecraft mods.

==> sn-sample-bib.tex <==
\begin{thebibliography}{9}

\bibitem{bib1} I.~Podlubny, Fractional Differential Equations, Academie Press, New York, 1999.

\bibitem{bib2} R. Hilfer, Application of Fractional Calculus in Physics, World Science Publishing, Singapore, 2000.

\bibitem{bib3} A. Nagih, G. Plateau, Fractional problems: overview of applications and solutions. Rairo-Recherche Operationnelle-Oper Press, New York, 1999.

\bibitem{bib4} J. P. Richard, Time-delay system: an overview of some recent advances and open problems, Automatica, 39(10) (2003) 1667-1694.

\bibitem{bib5} H. Ye, J. Gao, Y. Ding, A generalized Gronwall inequality and its application to a fractional differential equation, J. Math. Anal. Appl., 328 (2007) 1075-1081.

\bibitem{bib6} M. Lazarevic, Stability and stabilization of fractional order time delay systems, Scientific Technical Review, 61 (2011) 31-45.

\bibitem{bib7} Y. Li, Y. Q. Chen, I. Podlubny, Stability of fractional-order nonlinear dynamic systems: Lyapunov direct method and generalized Mittag-Leffler stability, Comp. Math. Appl., 59 (2010) 1810-1821.


\end{thebibliography}


